Rating transitions forecasting: a filtering approach

Analyzing the effect of business cycle on rating transitions has been a subject of great interest these last fifteen years, particularly due to the increasing pressure coming from regulators for stress testing. In this paper, we consider that the dynamics of rating migrations is governed by an unobserved latent factor. Under a point process filtering framework, we explain how the current state of the hidden factor can be efficiently inferred from observations of rating histories. We then adapt the classical Baum-Welsh algorithm to our setting and show how to estimate the latent factor parameters. Once calibrated, we may reveal and detect economic changes affecting the dynamics of rating migration, in real-time. To this end we adapt a filtering formula which can then be used for predicting future transition probabilities according to economic regimes without using any external covariates. We propose two filtering frameworks: a discrete and a continuous version. We demonstrate and compare the efficiency of both approaches on fictive data and on a corporate credit rating database. The methods could also be applied to retail credit loans.

==> Calibration.tex <==
\section{Calibration}
\label{sec:calibration}
In this section, we explain how to estimate model parameters involved in the filtering equations (\ref{eq:continuous-filter-rating}) and (\ref{eq:multivariate-discreet-credit}). We adapt the so-called Baum-Welch algorithm to our discrete-time and continuous-time framework. 
%In this section, we propose two adaptations of the classical HMM Baum-welch algorithm in order to use the parameter estimations in the filtering formulas (\ref{eq:continuous-filter-rating}) and (\ref{eq:discreet-credit-filter}). 
\subsection{A Baum-Welch algorithm adapted for a discrete framework}
The proposed method is a maximisation expectation (EM) algorithm for hidden Markov chains (HMM), adapted to the model. We can find studies on the classical model in \cite{Bishop2006}, \cite{Ozcan2013}, \cite{Rabinet1989} and \cite{Tenyakov2014}. 
\\
However the classical algorithm is not totally suitable for calibration of the discrete filtering equation (\ref{eq:multivariate-discreet-credit}).
We highlight two inconsistencies between the classical algorithm and our model:
\begin{itemize}
\item In HMM classical framework, rating status law is only governed by the state of the hidden factor. In the provided framework, it also depends on the previous rating.
\item Rating process trajectories of each entity must be independent whereas in our framework, they are dependent through the common factor $\Theta$.
\end{itemize}
The first step of the algorithm assigns initial values to the parameters we want to estimate. Then the algorithm replaces the missing data (states of $\Theta$) with Bayesian estimators using the observations and the current parameters estimated values.
\\
The second one consists in improving a conditional likelihood. Better parameters are estimated. Then these new estimates are used to repeat the first step. We iterate this process to converge to a local maximum.
%The values of parameters increase a like-hood and converge up to a local equilibrium at every step.
\\
\\
%Formally, in classical HMM algorithm, the future observation depends only on the state in which the unobserved process is. 
In the previous discrete-time framework, it is assumed that the jumps of $\Theta$ at time $n$ cannot directly affect rating process $Z$ at time $n$ (there should be a response time between). That's why, contrary to classical HMM models, we assume that the law of the rating process at current time $n$ is governed by the hidden factor $\Theta$ at the preceding time. Obviously, this consideration has no impact on the filtering. 
\\
As the new rating does not only depend on the economic cycle (state of $\Theta$) but also on the previous rating, we extend a classical version of the Baum-Welch algorithm by considering that 
\begin{equation}
\forall \ n \in [1,\Gamma]: \Prob(Z_{n}|Z_{0},...,Z_{n-1},\Theta_{0},...,\Theta_{n-1})=\Prob(Z_{n}|Z_{n-1},\Theta_{n-1}).
\end{equation}
Furthermore, as rating history of all entities are dependent on a same realization of $\Theta$, we must adapt our algorithm differently from \cite{oh2019estimation} who considered that each rating process is governed by its own and independent trajectory of $\Theta$.

\subsection{Initialization}
The calibration algorithm presented is based on iterative improvement of a likelihood. This expectation maximization algorithm (EM) (see \cite{dempster1977maximum}), as most of iterative maximisation algorithms, might be trapped in a local maximum. 
Obtained parameters may not be relevant when the global maximum is not found. This success is deeply dependant on the initialization.
%Indeed, the convergence to a point is deeply dependent of the initialization.
Several empirical and analytical methods have been proposed to deal with this matter. In \cite{liu2014proper}, transition probabilities are initiated using empirical frequencies. They succeed to considerably reduce the number of iterations to find their local maximum. By noticing that the transition matrices have strong diagonals, \cite{oh2019estimation} initialized their model by adding small perturbations to identity matrix or to uniform distributions.
In our study we choose a third option which seems to be more reliable: we test a high number of initial values (picked at random) in order to find the global maximum. 
%This intuition and its convergence are formalised and studied in \cite{Matar2021}. 
%The random choice of values has to be uniform to make the convergence almost surely.
In order to guarantee almost surely convergence to the global maximum, initial values are chosen according to a uniform distribution on the parameters space.
%However a uniform law cannot be defined on a space which has zero Lebesgue-measure: a model transfer to a smaller space dimension, a compact with no empty interior, is then achieved. 







\subsection{Bayesian estimators}
This part only presents the main results of the algorithm. Proofs and derivations of estimators are provided in Appendix (\ref{proof:calibration-discreet}).
\\
Let $Z=(Z^q)_{q}$ be the multivariate rating process and we call for $(n_1,n_2) \in \{0,\ldots,\Gamma\}^2$, $(Z)_{n\in [n_{1},n_2]}=Z_{n_{1}|n_{2}}$, the rating trajectories between time $n_1$ and $n_2$. We define the forward probability as denote,
%{\footnotesize
\begin{equation}
\forall s \in \T, \forall n \in \{1,\ldots,\Gamma\}: 
\alpha_{n}(s)=\Prob(Z_{0|n}=z_{0|n},\Theta_{n-1}=s)
\end{equation}
%}
and the backward probability as
\\
%{\footnotesize
\begin{equation}
\forall s \in \T, \forall n \in \{1,\ldots,\Gamma-1\}: 
\beta_{n}(s)=\Prob(Z_{n+1|\Gamma}=z_{n+1|\Gamma}|Z_{n}=z_{t},\Theta_{n-1}=s).
\end{equation}
%}
\\
We use the following recursive formulas in order to compute the two previous probabilities
%{\footnotesize
\begin{equation}
\label{alpha}
\alpha_{n}(s)=\sum_{l=1}^{m}\alpha_{n-1}(l)K^{ls}\prod_{d}L^{s,z_{n-1}^{d}z_{n}^{d}},
\end{equation}
%{\footnotesize
\begin{equation}
\label{beta}
\beta_{n}(s)=\sum_{l=1}^{m}\beta_{n+1}(l)K^{sl}\prod_{d}L^{l,z_{n}^{d}z_{n+1}^{d}}.
\end{equation}
For $n \in \{1,\ldots,\Gamma\}$, we introduce two random variables useful to describe $\Theta$
\\
%{\footnotesize
\begin{equation}
\label{u}
u_{n}(h)=\mathds{1}_{[\Theta_{n}=h]},
\end{equation}
\begin{equation}
\label{v}
v_{n}(s,h)=\mathds{1}_{[\Theta_{n}=h,\Theta_{n-1}=s].}
\end{equation}
%}
The forward and backward probabilities are helpful to compute the following Bayesian estimators 
\\
%{\footnotesize
\begin{equation}
\check{u}_{n}(h)=\Prob(\Theta_{n}=h|Z_{0|\Gamma}=z_{0|\Gamma})=\frac{\beta_{n+1}(h)\alpha_{n+1}(h)}{L_{\Gamma}},
\end{equation}
%}
and 
\begin{equation}
\check{v}_{n}(s,h)=\Prob(\Theta_{n}=h,\Theta_{n-1}=s|Z_{0|\Gamma}=z_{0|\Gamma})=\frac{\beta_{n+1}(h)K^{sh}\alpha_{n}(s)\prod_{d}L^{h,z_{n}^{d}z_{n+1}^{d}}}{L_{\Gamma}},
\end{equation}
where $L_{\Gamma}$ is the likelihood of the whole sample,
%{\footnotesize
\begin{equation}
L_{\Gamma}=\Prob(Z_{0|\Gamma}=z_{0|\Gamma})=\sum_{j}\alpha_{\Gamma}(j).
\end{equation}

\subsection{Parameters estimation}
The maximization phase consists in finding better parameters than those of the previous iteration.
We call $M^{(r)}=(\Pi^{(r)},L^{(r)},K^{(r)})$, the parameters obtained at the iteration $(r)$.
\\
%To compute the parameters at iteration (s+1), we define
%\\
%{\footnotesize
%\begin{equation}
%w_{i}=\Prob(Z,\Theta=\theta_{i}|M^{(s)}),
%\end{equation}
%\begin{equation}
%r_{i}=\Prob(Z,\Theta=\theta_{i}|M^{(s+1)}).
%\end{equation}
%\\
The new parameters are deemed to improve the likelihood according to: 
\begin{equation}
\Prob(Z|M^{(r+1)})\geq \Prob(Z|M^{(r)}).
\end{equation}
To achieve that, we are looking for maximizing $\log\frac{\Prob(Z|M^{(r+1)})}{\Prob(Z|M^{(r)})}$, which is equivalent to maximizing
\\
\\
%{\footnotesize
\begin{equation}
\begin{aligned}
Q(M^{(r)},M^{(r+1)})& =\sum_{i=1}^{m} \Prob(\Theta=i, Z|M^{(r)})\log(\Prob(\Theta=i,Z|M^{(r+1)}).\\
\end{aligned}
\end{equation}
%}
\\
After optimization, we obtain the following estimators
\\
%{\footnotesize
\begin{equation}
\begin{aligned}
\Pi_{h}=\check{u}_{0}(h),
\end{aligned}
\end{equation}
\\
\begin{equation}
\begin{aligned}
L^{h,ir}
& =\frac{\sum_{d}\sum_{n}\check{u}_{n}(h)\mathds{1}_{[z_{n}^{d}=r,z_{n-1}^{d}=i]}}{\sum_{d}\sum_{n}\check{u}_{n} (h)\mathds{1}_{[z_{n-1}^{d}=i]}},\\
\end{aligned}
\end{equation}
\\
\begin{equation}
\begin{aligned}
K^{sh}
& =\frac{\sum_{n}\check{v}_{n}(s,h)}{\sum_{n}\check{u}_{n-1}(s)}.\\
\end{aligned}
\end{equation}
%}
\\
\begin{proof} for more details, see Appendix (\ref{proof:calibration-discreet})
\end{proof}
\subsection{Continuous adaptation: compliance with discrete data}
\label{seq: continuous-adaptation}
This part aims to calibrate parameters involved in the continuous filtering formula (\ref{eq:continuous-filter-rating}). We propose an adaptation of the calibration algorithm in order to be compliant with the continuous filtering formula (\ref{eq:continuous-filter-rating}). Previous adaptations done for the discrete framework are still required but are not sufficient: Baum-Welch algorithm is an estimation in discrete time which is not compliant with the continuous version of the filter. Furthermore simultaneous jumps are forbidden when the processes are assumed to be continuous.\\
For the first deviation, we propose to realize the calibration in discrete time anyway. Then it is necessary to switch to continuous time dimension for filtering. The transition between probabilities to intensities turns out to be easy when the time interval chosen is small enough according to (\ref{K-to-k}) and (\ref{L-to-l}). 
\\
The second deviation is also essential and realistic: there is no common jumps among the rating processes. 
%This hypothesis mirrors the reality since any event occurs exactly at the same moment. 
However, ratings are not natural processes. Human decisions and algorithm appreciations are reported at the same moment in a day. Therefore we have to deal with simultaneous daily observations. 
%This part aims to present how we can use the continuous framework with multiple daily observations.  
\\
Our solution consists in considering a different time grid. Each day is cut into small intervals and jumps are randomly spread on these time intervals. We insure to cut enough finely to have a maximum of one jump per interval. This manipulation has two drawbacks. First, the conditional independence between rating entities might be lost if the non-simultaneity of jumps is enforced. Then, distributing simultaneous jumps on a finer time grid may ultimately modify the original information.
\\
The second effect is studied in a testing benchmark at (\ref{ContinuousFictive}).
\\
Once the data have been modified, we adapt our calibration algorithm to respect continuous structure. To this end, we use a prior law of jumps which respects the constraint of no simultaneity (that the number of observed jumps is only 0 or 1). 
%The following model insures that several entities can not jump at the same time. 
%\\
%Here, we only present the results of such an adaptation.
The main idea consists on assuming that one entity is randomly chosen to be allowed to jump. Then, the entity may jump according the common migration matrices $(L^{h,ir})_{h}$, $ (i,r) \in \{1,..,p\}$.
\\
%Let $n_{t}$ be the total number of entities at time t and $\bar{n}=\max_t n_{t}$ the maximum reached over the whole calibration time period.
%\\
%In order to make the model identifiable while considering the impact of the size of the sample (which may evolve), we define an independent process $I$, on $[0,\bar{n}]$, which chooses uniformly the entity which may jumps. 
%If $I$ picks an entity which is not in the current sample (because not already rated or censored...), we do not observe any jumps. Otherwise the entity can jump according to the transition matrices $(L^{h})_{h}$. 
%\\
%\\
%We have $\forall t \in [0,\Gamma],\ (j,k) \in (1,p)^2,\ h \in \T,\ q \in [0, \bar{n}]$
%\[\Prob(Z_{t}^q=k|Z_{t-1}^q=j,I_{t-1}=q,\Theta_{t-1}=h)=L^{h,jk}.\]
%With such assumption, the new transition probability can be expressed as
%\begin{equation}
%\label{eq:calibration-continuous}
%\begin{aligned}
%\Prob(Z_{t}=z_{t}|Z_{t-1}=z_{t-1},\Theta_{t-1}) =(1-\frac{n_{t-1}}{\bar{n}})\mathds{1}_{[z_{t}=z_{t-1}]} +\sum_{q=1}^{n_{t-1}}\frac{1}{\bar{n}}\mathds{1}_{[|z_{t}-z_{t-1}|_{0}\leq 1]}\mathds{1}_{[\forall l \neq q \ z_{t}^{l}=z_{t-1}^{l}]}L^{\Theta_{t-1},z_{t-1}^q,z_{t}^q},
%\end{aligned}
%\end{equation}
%where
%$|x|_{0}= \# \{x_{i}\neq 0\}$.
%\\
%\\
%To be compliant with the non simultaneity of jumps we adapt the previous algorithm by using the new expression (\ref{eq:calibration-continuous}) of $\Prob(Z_{t}=z_{t}|Z_{t-1}=z_{t-1},\Theta_{t-1})$, whenever the term appears in the computation of estimators. 
\\
More details of this adaptation can be found in Appendix \ref{proof:calibration-continuousBaum}.



==> ContinuousDerivation.tex <==
\section{Continuous-time version of the filter}
\label{sec:continuous-filter}
\subsection{Framework and statements}
\label{setting:continuous-filter}
Let $(\Omega,\bfA,\bfF = (\cF_t)_{t \in [0,T]},\Prob)\,,
$ be a filtered probability space satisfying the ``usual conditions'' of right-continuity and completeness needed to justify all operations to be made. All stochastic processes encountered are assumed to be adapted to the filtration $\bfF$ and integrable on $[0,T]$. In particular, we have $\bfA=\cF_{T}$.
The time horizon $T$ is supposed to be finite.
\\
\\
The problem is to estimate the states of an unobserved process $\Theta$ using only the information $ \bfF^N$, %\subset \bfF $,
resulting from the observation of a counting process $ N $.
We also define $\bfF^{\Theta}$, the natural filtration of $\Theta$. 
By definition of the conditional expectation,
\[\hat{\Theta}_t = \E [\Theta_t | \cF_t^N]\,.
\]
is the $L^2$ approximation of $\Theta$ knowing N.
With the same notation, all the processes O filtered  by $ \cF_t^N $ are written 
\[\hat{O}_t = \E [O_t | \cF_t^N].\]
Unfortunately, the explicit computation of $\hat{\Theta}$ (by the Bayes formula) is only possible in very simple cases, for example, when $ N$ is a mixture of Poisson processes. Moreover, numerical approaches are extremely heavy to implement as soon as non-trivial models are considered.
\\
The filtering approach is different. It consists in writing $\hat{\Theta}$ as the solution of a stochastic differential equation (SDE). 
%\subsection{Filtering univariate point process}
%\subsection{Filtering univariate point process}
The main result on univariate point process filtering can be stated in the following way (see \cite{Bremaud1981}, \cite{Karr1991}, \cite{Leijdekker_Spreij2008}, \cite{vanSchuppen1997}). 
\begin{proposition}
\textit{
Let $\Theta$ be a process of the form 
$$
d \Theta_t = a_t \, \diff t + \diff M_t \,,
$$
where $ M $ is a martingale with no jumps in common with $ N $. Then, the process $\hat{\Theta}$ satisfies the following equation
\begin{equation}
\diff \hat{\Theta}_t = \hat{a}_t \, \diff t + \eta_t \, (\diff N_t - \hat{\nu}_{t-} \, \diff t)\,,
\label{eq:discreet-univariate-filter}
\end{equation}
with
\begin{equation}
\eta_t = \frac{\widehat{(\Theta \,\nu)}_{t-}}{\hat{\nu}_{t-}} - \hat{\Theta}_{t-} \,,        
\end{equation}
and where $\nu$ is the $\bfF$-intensity of $N$.}
\end{proposition}
\begin{proof} 
see \cite{Bremaud1981}
\end{proof} 
In order to study the dynamics of ratings in a credit portfolio or the dynamics of rating migrations, this filtering equation must be extended to a multivariate case.
\subsection{Filtering multivariate point process}
In this section, we show that the previous filtering equation admits a natural multivariate extension.
Let $N = (N^1, \ldots, N^\rho)$ be a multivariate counting process where $N^j=(N_t^j)_{t \in [0,T]}$, $j=1, \ldots, \rho, $ is a set of
simple counting processes, such that,
$N_t^j =\sum_{0<s \leq t} \Delta N_s^j< \infty$ and $\Delta N_s^j \in \{0,1 \}$, for any $j=1, \ldots, \rho$. It is assumed that these processes admit a predictable $\bfF$ - intensity
$\nu^j =(\nu_t^j)_{t\in [0,T]},$ and that they do not have any common jumps, i.e.,  $\Delta N_t^j \Delta N_t^k =\delta_{jk}\Delta N_t^j$ ie $[N^j,N^k]_{t}=0$ (the continuous martingale part of a counting process being null).  We introduce $\bfF^N = (\cF_t^N)_{t \in [0,T]}$ the natural filtration of the multivariate counting process $N=(N^1,...,N^\rho)$.
\begin{proposition}
\label{Prop:filtering_multPP}
\textit{Let $\Theta$ be a square integrable process of the form}
\begin{equation}
\Theta_t = \int_0^t a_s \, \diff s + M_t \,,
\label{eq:Theta_t}
\end{equation}
\textit{where $a$ is a $\bfF$-adapted process and $M$ is a $\bfF$-square integrable martingale with no jumps in common with $N$. Therefore, the process $\hat{\Theta}$ is solution of the SDE}
\begin{equation}
\diff \hat{\Theta}_t = \hat{a}_t \, \diff t + \sum_j \eta_t^j \, (\diff N_t^j - \hat{\nu}_{t-}^j \, \diff t)\,,
\label{eq:dhatTheta}
\end{equation}
\textit{with}
\begin{equation}
\eta_t^j = \frac{\widehat{(\Theta \,\nu^j)}_{t-}}{\hat{\nu}_{t-}^j} - \hat{\Theta}_{t-} \,,
\label{eq:eta^j}
\end{equation}
\textit{and initial condition}
\begin{equation}
\hat{\Theta}_0 = \E [\Theta_0] \,.
\label{eq:hatTheta_0}
\end{equation}
\end{proposition}
\begin{proof}
 Let $g$ and $h$ be two $\bfF$ predictable processes such that $\E \left[ \int_0^T (g_s^2+ h_s^2)  \, \nu_s^j \, \diff s \right] \leq \infty$. We introduce the processes $X$ and $Y$ defined by
%In particular, the martingales in (\ref{eq:compensated-N}) are square integrable and mutually orthogonal.
%\\
%The heuristics of these definitions and results are as follows. Interpreting $\diff N_t^j$ as the number of jumps of $N^j$
%*** say 0 or one
%in the small time interval $[t,t+\diff t)$,
%\begin{equation}
%\Prob [\diff N_t^j = 1 | \cF_{t-}] = 1 - \Prob [\diff N_t^j = 0 | \cF_{t-}] = \E [\diff N_t^j | \cF_{t-}] = \nu_t^j \, \diff t \,,
%\label{eq:Def-nu}
%\end{equation}
%all equalities up to a negligible term $o(\diff t)$. The martingale property (\ref{eq:tiN-mg}) follows from
%\begin{align*}
%\E \left[ N_u^j - N_t^j - \int_t^u \nu_s^j \, \diff s \,|\, \cF_t \right] =
%\E \left[ \int_t^u \E (\diff N_s^j - \nu_s^j \, \diff s) | \cF_{s-} ) \,|\, \cF_t \right] = 0 .
%\end{align*}
%As the increments $\diff N_t^j$ are binary and at most one of them can be 1, $\diff N_t^j \, \diff N_t^k = \delta_{jk} \diff N_t^j$, hence
%$$
%\E [\diff N_t^j \, \diff N_t^k | \cF_{t-}] = \delta_{jk} \, \nu_t^j \, \diff t \,.
%$$
%This entails orthogonality of the martingales in (\ref{eq:compensated-N}):
%\begin{align*}
%\begin{aligned}
%\E [(\diff N_t^j - \nu_t^j \, \diff t) (\diff N_t^k - \nu_t^k \, \diff t)| \cF_{t-}] = & 
%\E [\diff N_t^j \, \diff N_t^k | \cF_{t-}]
%- \nu_t^j \, \diff t \, \E [ \diff N_t^k | \cF_{t-}] 
%- \E [ \diff N_t^j | \cF_{t-}] \, \nu_t^k \, \diff t + \nu_t^j \, \diff t \, \nu_t^k \, \diff t  \\
%= & \delta_{jk} \, \nu_t^j \, \diff t + o(dt)\,.  
%\end{aligned}
%\label{eq:orthog}
%\end{align*}
%Finally, (\ref{eq:EintNjintNk}) is obtained upon rewriting the expression on the left as (Fubini and iterated expectation)
%\begin{equation}
%\E \left[ \left. \int_t^T \int_t^T \E [ g_r \,(\diff N_r^j - \nu_r^j \, \diff r)  \, h_s \, (\diff N_s^k - \nu_s^k \, \diff s) \,|\, \cF_{\max(r,s)-}] \, \right| \, \cF_t \right]
%\label{eq:integrand}
%\end{equation}
%and observing that diagonal terms ($r = s$) under the integral reduce to $\delta_{jk} \, g_s \, h_s \, \nu_s^j \,\diff s$ due to (\ref{eq:orthog}), and that off-diagonal terms vanish: e.g. for any $r < s$ it is
%$$
%g_r \,h_s \, (\diff N_r^j - \nu_r^j \, \diff r) ( \E [\diff N_s^k | \cF_{s-}] - \nu_s^k \, \diff s) = 0 \,.
%$$
$X_t=\int_0^t g_{r} (\diff N_r^j - \nu_r^j \, \diff r)$ and $Y_{t}=\int_0^t h_s (\diff N_s^k - \nu_s^k \, \diff s)$ for all $t \le T$. X and Y are two $\bfF$--martingales.
The Itô formula applied to $XY$ yields 
\begin{align*}
\label{int-part}
\diff(X_tY_t) = & X_{t-}\diff Y_{t} + Y_{t-}\diff X_{t} + \Delta X_t \Delta Y_{t}.
\end{align*}
Since $N^j$ and $N^k$ have no common jumps,
$
\Delta X_t \Delta Y_{t}=g_{t}h_{t}\Delta N_{t}^j \delta_{jk}.
$
Then,  we obtain
\begin{equation}
\label{eq1}
\E[X_{T}Y_{T}- X_{t}Y_{t}|\cF_{t}]=\delta_{jk}\E\left[\int_{t}^T g_{s}h_s
\diff N^j_{s} |F_{t}\right].
\end{equation}
Note that $X_T Y_T-X_t Y_t=(X_{T}-X_{t})(Y_{T}-Y_{t})-2X_{t}Y_{t}+X_{t} Y_{T} + X_{T} Y_{t}$. Then, 
\begin{equation}
\label{eq2}
\E[X_{t}Y_{T}-X_{t}Y_{t}|\cF_{t}]=\E[(X_{T}-X_{t})(Y_{T}-Y_{t})|\cF_{t}].
\end{equation}
Note that the process $Z=\left(\int_{0}^t g_{s}h_{s}(\diff N^j_{s}-\nu^j_{s}\diff{s})\right)_{0 \le t \le T}$ is a $\bfF$--martingale.
\\ 
So, $\E\left[Z_{T}-Z_{t}|\cF_{t} \right]=0$. Combining this remark with Equations~\eqref{eq1} and \eqref{eq2}, we finally obtain \begin{equation}
\E \left[ \left. \int_t^T g_r (\diff N_r^j - \nu_r^j \, \diff r) \int_t^T h_s (\diff N_s^k - \nu_s^k \, \diff s) \right| \cF_t \right] = \delta_{jk} \, \E \left[ \left. \int_t^T g_s h_s \, \nu_s^j \, \diff s \right| \cF_t \right] .
\label{eq:EintNjintNk}
\end{equation}
The innovation theorem says that the $\bfF^N$-intensities of the counting processes $N^j$ exist and are
\begin{equation}
\hat{\nu}_{t-}^j =\E \left[ \nu_{t-}^j \,|\, \cF_{t-}^N \right] =\E \left[ \nu_{t}^j \,|\, \cF_{t-}^N \right] \,.
\label{eq:innovation-rule}
\end{equation}
%This follows by the tower property of conditional expectation applied to the heuristic definition (\ref{eq:Def-nu}) of the intensity:
%$$
%\E [\diff N_t^j \,|\, \cF_{t-}^N] = \E [\, \E [\diff N_t^j | \cF_{t-}] \,|\, \cF_{t-}^N] = \E [ \nu_t^j \, \diff t \,|\, \cF_{t-}^N]
%= \E [ \nu_{t-}^j \,|\, \cF_{t-}^N] \, \diff t
%$$
%\ares{(left-limits are of no significance in the presence of the factor $\diff t$)}.
For any $\bfF^N$ predictable process $h$ satisfying $\E\left[\int_0^T |h_s \nu_s| ds \right]< \infty$, we have
\begin{align*}
\E \left[\int_{0}^{\infty} h_{t}\diff N_{t}\right]
=& \E \left[\int_{0}^{\infty} h_{t}\nu_{t} \diff t \right]
= \E \left[\int_{0}^{\infty} h_{t}\E \left[\nu_{t}|\cF^N_{t-}\right] \diff t\right]
= \E\left[\int_{0}^{\infty} h_{t}\hat{\nu}_{t-} \diff t\right].
\end{align*}
Now, rewrite (\ref{eq:Theta_t}) as
\begin{equation}
\Theta_t = \int_0^t \hat{a}_s\, \diff s + L_t + M_t \,,
\label{eq:Theta-rewrite}
\end{equation}
with
\begin{equation}
L_t = \int_0^t (a_s - \hat{a}_s)\,ds  \,.
\label{eq:M^*}
\end{equation}
Taking conditional expectation, w.r.t. $\cF_t^N$, in (\ref{eq:Theta-rewrite}) yields
\begin{equation}
\hat{\Theta}_t = \int_0^t \hat{a}_s\,ds + \hat{L}_t + \hat{M}_t \,.
\label{eq:hat-Theta-repr}
\end{equation}
While $L$ need not be a $\bfF$--martingale, it is clear that $\hat{L}$ is an $\bfF^N$--martingale. For $r < t$,
%*** Proof reallly needed?
\begin{align*}
 \E [ \hat{L}_t - \hat{L}_r  \,|\, \cF_r^N ]
 &=& \E \left[ \left. \int_r^t \left( a_s - \E [ a_s | \cF_s^N ] \right) \,\diff s \right| \cF_r^N \right]=0. \\
\end{align*}
From the tower property, we deduce that $\hat{M}$ is also a $\bfF^N$--martingale.
% \begin{align*}
% \E [\hat{M}_t \,|\, \cF_r^N] &=& \E [\, \E [M_t | \cF_t^N] \,|\, \cF_r^N] = \E [M_t | \cF_r^N] = \E [\, \E [M_t | \cF_r] \,|\, \cF_r^N] \\
% &&= \E [M_r| \cF_r^N]
% =  \hat{M}_r .
% \end{align*}
Introduce
\begin{equation}
K_t = L_t + M_t = \Theta_t - \int_0^t \hat{a}_s\,ds \,.
\label{eq:K}
\end{equation}
Since $\Theta$ and $N$ have no common jumps, we can deduce that $K$ and $N$ have any either. 
It has been shown that $\hat{K}= \hat{L} + \hat{M}$ is a $\bfF^N$--martingale. Therefore it has a predictable representation,
\begin{equation}
\hat{K}_t = \ga + \sum_j \int_0^t \eta_s^j \, (\diff N_s^j - \hat{\nu}_{s-}^j \, \diff s) ,
\label{eq:pred-repr}
\end{equation}
where $\ga = \hat{K}_0$ is $\cF_0^N$-measurable and the $\eta^j$ are $\bfF^N$-predictable processes (see \cite{Bremaud1981}). Note that $\hat K_0 = \E[\Theta_0]$.
Now, any integrable $\bfF^N$-measurable random variable has a representation $g + \sum_j \int_0^t h_s^j \, (\diff N_s^j - \hat{\nu}_s^j \, \diff s)$, with $g$ constant and the $h^j$ are $\bfF^N$-predictable. Therefore, since $\hat{K}_t$ is the $L^2$ projection of $K_t$ onto the space of square integrable $\cF_t^N$-measurable random variables, the coefficients in the representation (\ref{eq:pred-repr}) are uniquely determined by the normal equations
$$
\E \bigg[ \bigg( K_t - \ga - \sum_j \int_0^t \eta_s^j (\diff N_s^j - \hat{\nu}_{s-}^j \, \diff s) \bigg) \bigg( g + \sum_j \int_0^t h_s^j (\diff N_s^j - \hat{\nu}_{s-}^j \, \diff s)  \bigg) \bigg] = 0,
$$
for all constants $g$ and all $\bfF^N$-predictable processes $h^j$.  Setting $g = 0$ and using (\ref{eq:EintNjintNk}) give
\begin{equation}
\label{eq:inserting}
\E \left[ K_t \, \sum_j \int_0^t h_s^j \, (\diff N_s^j - \hat{\nu}_{s-}^j \, \diff s) -
\sum_j h_s^j \, \eta_s^j \, \hat{\nu}_{s-}^j \, \diff s   \right] = 0 \,.
\end{equation}
For j $\in \{1, \dots,\rho\}$, we compute $\E \left[K_{t}\int_0^t h_s^j \diff N_s^j \right]$. Using that $\hat K$  is a $\bfF^N$--martingale and that $K$ and $N^j$ have no common jumps, we have
\begin{align*}
\begin{aligned}
\E \left[K_{t}\int_0^t h_s^j \diff N_s^j \right]
= & \E \left[K_{t}\sum_{s \leq t} h_s^j \Delta N_s^j \right]
= \sum_{s \leq t}\E \left[\E\left[K_{t}|\cF_{s}^N \right] h_s^j \Delta N_s^j \right]\\
= & \sum_{s \leq t}\E \left[\hat{K}_{s} h_s^j \Delta N_s^j \right] = \E \left[\int_0^t  K_{s-}h_{s}^j \diff N_s^j \right]\\
= & \E \left[\int_0^t K_{s-}h_{s}^j \nu_s^j \diff{s} \right]
=  \int_0^t \E \left[h_{s}^j \E\left[ K_{s-} \nu_s^j| \cF_{s-}^N \right] \right] \diff{s}\\
= & \E \left[\int_{0}^t h_{s}^j \widehat{\Theta \nu^j}_{s-} \diff s \right] - \E \left[\int_{0}^t h^j_{s} \hat{\nu}_{s-}^j\int_{0}^s \hat{a}_{u}\diff u  \ \diff s \right].
\end{aligned}
\end{align*}
Using similar arguments, we compute the second term 
\begin{align*}
\begin{aligned}
\E \left[K_{t}\int_{0}^t h^j_s \hat{\nu}^j_{s-} \diff s\right]
= &  \int_{0}^t \E \left[ h^j_s \E \left[{K}_{t}|\cF_{s-}^N\right]  \hat{\nu}^j_{s-} \right]\diff s 
=  \int_{0}^t \E \left[ h^j_s \hat{K}_{s-}  \hat{\nu}^j_{s-} \right]\diff s \\
%= & \int_{0}^t \E \left[ \E \left[ h^j_s \hat{K}_{t} \hat{\nu}^j_{s-}|\cF_{s-}^N \right] \right]\diff s\\
%= &( \hat{K} \ is \ a  \ \cF^N \ martingale)\\
%= & \E\left[\int_{0}^t h^j_s \hat{K}_{s-}\hat{\nu}^j_{s-} \diff s \right]\\
= & \E\left[\int_{0}^t h^j_s \hat{\Theta}_{s-}\hat{\nu}^j_{s-} \diff s \right] - \E\left[\int_{0}^t h^j_s \hat{\nu}^j_{s-} \int_{0}^s\hat{a}_{u} \diff u \ \diff s \right]. 
\end{aligned}
\end{align*}
Inserting these expressions into (\ref{eq:inserting}), gives
\begin{align*}
\sum_j \E \left[ \int_0^t h_s^j \left( \widehat{\Theta\, \nu^j}_{s-} - \hat{\Theta}_{s-} \, \hat{\nu}_{s-}^j - \eta_s^j \,\hat{\nu}_{s-}^j \right) \, \diff s  \right] = 0.
\end{align*}
Choosing $h_s^j$ equal to the expression in the parentheses, gives $\sum_j \E \left[ \int_0^t (h_s^j)^2 \, \diff s  \right] = 0$ hence all $h^j$ vanish and $\forall \ j = 1,\ldots,\rho$:
\begin{equation}
\eta_s^j = \frac{ \widehat{ \Theta_{s-}\,\nu_{s-}^j } } { \hat{\nu}_{s-}^j} - \hat{\Theta}_{s-}.
\label{eq:eta}
\end{equation}
From (\ref{eq:pred-repr}), (\ref{eq:hat-Theta-repr}), and the equality $\hat{K} = \hat{L} + \hat{M}$, it follows that
$$
\hat{\Theta}_t = \E[\Theta_0] + \int_0^t \hat{a}_s\, \diff s + \sum_j \int_0^t \eta_s^j \, (\diff N_s^j - \hat{\nu}_{s-}^j \, \diff s)
$$
with the $\eta^j$ are given by (\ref{eq:eta}). 
%In the latter $\widehat{ \Theta_{s-}\,\nu_{s-}^j }$ can be replaced with $\widehat {(\Theta \, \nu^j) }_{s-}$ due to dominated convergence. 
This finishes the proof of the proposition. \hfill
\end{proof}

\subsection{Finite latent factor model and a credit risk application}
\label{sec:rating-continuous}
This section aims to apply previous filtering framework to credit rating migrations.
In order to remain realistic and to fix the terminology, a bond market containing a finite number of individual bonds is considered. All bonds are affected by variable and random market conditions represented by the same latent process $\Theta$. 
A bond $q$ of the sample is observed between the dates $s^q$ and $u^q$, $0 \leq s^q \leq u^q \leq T$. At all times, the bond can only be in a state belonging to a finite set of states, $\J = \{1, \ldots, p \}$. This space represents different credit risk scores or ratings in descending order, $p$ being the default state. For example, Standard and Poor's long-term investment ratings can be translated to AAA = 1, AA = 2, A = 3, BBB =4, ..., D (Default) = 10.
\\
Let us define $\tilde{\J}=\{(j,k) \in \J^2,\  j \neq k\}$, the space of possible migrations.
Let $Z_t^q \in \J$ be the state of  bond $q$ at time $t$ and $Z^q = (Z_t^q)_{t \in [s^q,u^q]}$ be 
the rating process describing its evolution. The migration counting process associated with $Z^q$, which counts the number of jumps of the entity $q$ from rating $j$ to $k$, is denoted by $N^{q,jk}$ and is such that, $\forall t \in [s^q,u^q]$,
%\begin{equation}
%  N_t^{q,jk} = \sharp \{ s \in [0,t]; Z_{s-}^q = j, \, Z_s^q = k \},\ (j,k) \in \tilde{\J} .
%\end{equation}
\begin{equation}
\Delta N_{t}^{q,jk}=\mathbf{1}_{[Z_{t-}^q = j, Z_t^q = k]}.
\end{equation}
In this study, we assume that $(Z_{t}^q, t\in[0,T])_q$ are described within a  factor  migration model. 
More specifically, knowing $\cF_T^{\Theta}$, the rating processes $Z^q$ are assumed to be conditionally independent Markov chains 
with the same generator matrix.
%of each individual at time t, $Z_t^q$, are identically distributed and conditionally independent, knowing $\cF_t^{\Theta}$.\\
In reality the change of rating of a bond may also induce the change of state of other bonds but this contagion effect is not considered in this paper. Moreover, the censorship mechanism governing $(s^q, u^q)$ is assumed to be non-informative and can therefore be considered deterministic and belonging to $\cF_0^N$.
%Note that rating processes $(Z_{t}^q, t\in[0,T])_q$ are exchangeable. 
Under this exchangeable setting, to infer information on the underlying hidden factor $\Theta$, it is sufficient to observe the aggregated counting processes $N^{jk}$,  $(j,k) \in \ \tilde{\J}$,  defined by
\begin{equation}
N_t^{jk} = \sum_q N_t^{q,jk}.
\end{equation}
%governed by the $\bfF$ intensities $(\nu_t^{jk})_{(j,k) \in \tilde{\J}}$. 
and the exposure processes $Y^j$, $j \in  \J$ defined by
\begin{equation}
Y_t^j = \sum_{q;\, s^q \leq t < u^q}\, \mathbf{1}_{[Z_t^q =j]} \,.
\end{equation}
Note that the exposure process $Y^j$ is left continuous. It increases by 1 when  $N^{kj}$  jumps for any $k \neq j$, or when a new bond enters the pool with rating $j$. It decreases by 1 when a bound jumps outside rating $j$, i.e., whenever $N^{jk}$ jumps for $k\neq j$ or when a bond expires with rating $j$.
\\
We will now consider the filtering problem of $\Theta$ given observation of the multivariate processes $N:=(N^{jk}$,  $(j,k) \in \ \tilde{\J})$, using Prop. \ref{Prop:filtering_multPP}. We denote by $(\nu_t^{jk})_{(j,k) \in \tilde{\J}}$ the $\bfF$ intensity of $N$.
The dynamic (\ref{eq:dhatTheta}) suggests a recursive algorithm to update the process $\hat{\Theta}$. A consequence of (\ref{eq:dhatTheta}) is that the dynamics of $\hat{\Theta}$ depends on $\widehat{(\Theta \nu)}$ which in turn depends on the term $\widehat{(\Theta \nu^2)}$, and so on... This filtering equation induces an infinite nesting problem.\\
To solve the issue of infinite imbrication, we assume that the intensities $(\nu^{j,k})_{(j,k) \in \tilde{\J}}$ are governed by a finite state  Markov chain. Consequently the hidden factor driving process $\Theta$ is assumed to be a Markov chain with finite number of states  in $\T = \{1,\ldots,m\}$ and with constant transition intensities $k^{hi}$, $i \neq h$, such that $k^{hh} = - \sum_{i; i \neq h} k^{hi}$ and for small enough dt
%\begin{equation}
%\label{K-to-k}
%\forall \ i \neq h \in [1...m] :\Prob (\Theta_{t+dt} = h\,|\, \Theta_t = i) = k^{ih}\, dt + o(dt).
%\end{equation}
\begin{equation}
\label{K-to-k}
\forall \ i \neq h \in \T^2 :\Prob (\Theta_{t+dt} = h\,|\, \Theta_t = i) \approx k^{ih}\, dt.
\end{equation}
The initial distribution of $\Theta$ is defined
\begin{equation}
\forall i \in \T : \Pi_{i}=\Prob(\Theta_{0}=i).
\end{equation}
Let us introduce the processes $I^h$, $h \in \T$, defined by
\begin{equation}
I_t^h = \mathds{1}_{[\Theta_t = h]}, \; h \in \T.
\end{equation}
The process $\Theta$ can be represented as a finite sum of indicator processes
\begin{equation}
\Theta_t = \sum_{h \in \T} \, h\, I_t^h \,.
\label{eq:Theta-repr}
\end{equation}
With these assumptions, the processes $(Z^q)_q$ are governed as described before by their common intensity matrices $(l^h)_{h \in \T}$, such as for small enough dt
%\begin{equation}
%\label{L-to-l}
%\Prob [Z_{t+dt}^q = k\,|\, \Theta_t = h, Z_t^q = j ] = \ell^{h,jk}\, dt + o(dt).
%\end{equation}
\begin{equation}
\label{L-to-l}
\Prob [Z_{t+dt}^q = k\,|\, \Theta_t = h, Z_t^q = j ] \approx \ell^{h,jk}\, dt.
\end{equation}
Then the counting processes $N^{jk}$ are governed by the $\bfF$ intensities
\begin{equation}
\nu_t^{jk} = Y_t^j \, \sum_h \ell^{h,jk}\, I_{t-}^h \,.
\end{equation}
%Recall that $I_{t-}^{h}$ is the indicator function of the unobserved factor that is equal to 1 when the factor is in state $h$. \\
As $Y^{j}$ is $\bfF^N$--adapted, the $\bfF^N$--intensity of $N$, the counting process which counts the cumulative number of transitions, may be written 
\begin{equation}
\label{sigmaFil}
\hat{\nu}_{t-}^{jk} = Y_t^j \, \sum_h \ell^{h,jk}\, \hat{I}_{t-}^h \,,
\end{equation}
By applying the previous multivariate filtering formula (\ref{eq:dhatTheta}) to the process $(I_{t})_{t\in[0,T]}$, we obtain the following proposition. 
\begin{proposition}
\textit{
With the previous assumptions, the unobserved indicator process  filtered with rating jumps satisfies the following recursive equation}
\begin{equation}
d\hat{I}_{t}^{h}=\sum_{i=1}^{m}k^{ih}\hat{I}_{t-}^{i}dt+\hat{I}_{t-}^{h}\sum_{j\neq k}\left(\frac{l^{h,jk}}{\sum_{r}l^{r,jk}\hat{I}_{t-}^{r}}-1\right)\left(dN_{t}^{jk}-Y_{t}^{j}\sum_{i=1}^{m}l^{i,jk}\hat{I}_{t-}^{i}dt\right)
\label{eq:continuous-filter-rating}
\end{equation}
\end{proposition}
\begin{proof}
In order to apply Prop. \ref{Prop:filtering_multPP}, one needs to find the representation (\ref{eq:Theta_t}) for $I_t^h$. 
Let $\Psi^{hi}$, $h \neq i$, $h,i \in \T$, be the counting processes defined by
\begin{align*}
\Psi_t^{hi} = \sharp \{ s \in (0,t];\, \Theta_{s-} = h, \, \Theta_s = i \}\,.
\end{align*}
The starting point is the expression
\begin{align*}
I_t^h = I_0^h + \sum_{i; i \neq h} (\Psi_t^{ih} -  \Psi_t^{hi}) \,,
\label{ThetaIndicator}
\end{align*}
which comes from the obvious dynamics
\begin{align*}
dI_t^h = \sum_{i; i \neq h} (\diff \Psi_t^{ih} - \diff \Psi_t^{hi})
\end{align*}
The counting processes $\Psi^{hi}$ have intensities of the form $I_{t-}^h \, \ka^{hi}$. Reshaping the last expression as
\begin{align*}
I_t^h &=& I_0^h + \int_0^t \sum_{i; i \neq h} ( I_{s-}^i \, \ka^{ih} - I_{s-}^h \, \ka^{hi} ) \, \diff s \\
&&+ \int_0^t \sum_{i; i \neq h} \left[ (\diff \Psi_s^{ih} - I_{s-}^i \, \ka^{ih}\, \diff s)  - (\diff \Psi_s^{hi} - I_{s-}^h \, \ka^{hi} \, \diff s ) \right],
\end{align*}
shows that $I^h$ is of the form
\begin{align*}
I_t^h = \int_0^t a_s^h \, \diff s + M_t^h \,,
\end{align*}
with
\begin{equation}
a_t^h = \sum_{i; i \neq h} ( I_{t-}^i \, \ka^{ih} - I_{t-}^h \, \ka^{hi} ) = \sum_i \ka^{ih} \, I_{t-}^i
\label{eq:a}
\end{equation}
and $M^h$ is a martingale commencing at $M_0^h = I_0^h \,.$ This martingale has no jumps in common with $N$.
\\
Now, let $I^h$ take the role of $\Theta$ in Prop. \ref{Prop:filtering_multPP}. Then the role of $a_t$ is taken by $a_t^h$ in (\ref{eq:a}), the role of $(\Theta \, \nu^{j})_{t-}$ is taken by 
\begin{align*}
(-I^h\nu^{jk})_{t-}=I_{t-}^h \, Y_t^j \, \sum_i \ell^{i,jk} \, I_{t-}^i = Y_t^j \, \ell^{h,jk} \, I_{t-}^h \,,
\end{align*}
and the $\bfF^N$-intensities of $N$ are given in (\ref{sigmaFil}).
%\begin{align*}
%\hat{\nu}_t^j = Y_t^j \, \sum_i \ell^{i,j} \, \hat{I}_t^i \,.
%\label{eq:hatnu-multiplic}
%\end{align*}
Inserting these expressions
%*** reword
into (\ref{eq:dhatTheta}), gives
\begin{equation}
d\hat{I}_{t}^{h}=\sum_{i=1}^{m}k^{ih}\hat{I}_{t-}^{i}dt+\hat{I}_{t-}^{h}\sum_{j\neq k}\left(\frac{l^{h,jk}}{\sum_{r}l^{r,jk}\hat{I}_{t-}^{r}}-1\right)\left(dN_{t}^{jk}-Y_{t}^{j}\sum_{i=1}^{m}l^{i,jk}\hat{I}_{t-}^{i}dt\right)
\end{equation}
\end{proof}

\begin{remark}
%\subsection{Analyses of the filter}
%In this filtering formula (\ref{eq:continuous-filter-rating}), parameters are unknown:
%initial distribution  $(\Pi_{i})_{i}$, transition intensities of $\Theta$, $(k^{ij})_{i,j}$ and conditional transition intensities of the observable rating process $(l^{h,ij})_{h,i,j}$. In order to apply this formula, we need to estimate these parameters. An important purpose of this study consists on seeking a way to calibrate them.
Despite being non-linear, the filtering equations (\ref{eq:continuous-filter-rating}) can be decomposed into a prediction term and an innovation term, as for the classical Kalman filter. Indeed, one can show that:
\begin{subequations}
\label{eq:Kalman}
\begin{align}
\E[I_{t}^{h}|F_{t-}^{N}]& =\hat{I}_{t-}^{h} +\sum_{i}k^{ih}\hat{I}_{t-}^{i}dt \label{eq:pred} \\
\E[I_{t}^{h}|F_{t}^{N}]& =\underbrace{\E[I_{t}^{h}|F_{t-}^{N}]}_{prediction}+\hat{I}_{t-}^{h}\sum_{j\neq k}\left(\frac{l^{h,jk}}{\sum_{r}l^{r,jk}\hat{I}_{t-}^{r}}-1\right)\underbrace{\left(dN_{t}^{jk}-Y_{t}^{j}\sum_{i}l^{i,jk}\hat{I}_{t-}^{i}dt\right)}_{new \ Information} \label{eq:corr}
\end{align}
\end{subequations}
%\underline{Proof}: See Appendices (\ref{proof:kalman}).
We can identify (\ref{eq:pred}) as the prediction term  and (\ref{eq:corr}) as the correction term.\\
%According to this decomposition, it would be possible to estimate the parameters using extended Kalman filter. Derivations of such extensions can be found in \cite{Ribeiro2004} but turns out to be very heavy.  Therefore we will focus on another alternative, described in  (\ref{seq: continuous-adaptation}).
\end{remark}
Usually, information on rating migrations are only available to public on a daily basis. For large credit portfolios, it is then frequent to observe multiple transitions (of several entities) occurring at the same day. In addition, clustering of rating migrations may also happen following the disclosure of a major economic events. Then, the presented continuous-time filtering approach is not fully compliant with migration data since it precludes simultaneous jumps. This has prompted us to develop an alternative discrete-time version of the filter. 


%Nevertheless our approach is not totally compliant with credit rating environment. %Ratings are not natural processes but based on human judgement:



%\subsection{Compliance with discreet data}
%Rating transitions are daily discreet data. Indeed data format does not allow to know the precise moment of a jump during a day. \\
%This constraint leads to simultaneous observations that is not consistent with continuous framework. 
%To solve this issue, we decide to spread randomly the information along the days. We cut each day in 1000 times intervals and then attribute randomly the daily jumps between those small intervals.
%This action let the hidden factor evolving.
%The purpose of this operation is multiple: 
%We make compliant the continuous model with discreet data. The advantage of using continuously observed data when estimating probabilities of unobserved or rare transitions as specifics rating transitions was observed in \cite{lando2002analyzing}: 
%The continuous framework is also more adapted to analyse the dependence's with external covariates, and changes in ‘regimes’ either due to business cycles can be quantified.
%\\
%Plus applying the model on gradually data decrease considerably the dimension of the model. 
%The consequences of such spread would be observed and analysed later in this paper.
%\\
%Nevertheless it would be more consistent to stay in the same setting throughout the framework. Therefore two adaptations are possible in order to overcome this issue: working with a continuous-time version of the EM algorithm or developing a discrete-time version of the filtering formula.
%Designing a continuous-time version of the EM algorithm is more involved since the hidden factor can jump at any time between two observations.
%\ares{the freedom the hidden factor has to jump at any time must be taken into account. A reformuler}
%We can find such extensions in \cite{nodelman2012expectation} and \cite{liu2017learning}. The latter papers introduce  computational methods, called the "Eigen" and "Expm" methods, that make the learning phase more efficient.
%One uses the eigen decomposition of matrices 
%Nevertheless the presence of common jumps in the data is still an issue  with these continuous-time extension of the EM algorithm.
%Therefore, we will focus on the second adaptation, i.e., developing a discrete-time version of the point process filtering formula in order to be more consistent the nature of the data.


==> Introduction.tex <==
\section{Introduction}

Credit risk research has been on the rise over the last 20 years. In particular, the challenges that arose from the previous financial crisis prompted researchers to develop credit risk valuation models that take into account the evolution of the business cycle. The evolution of the banking supervisor regulations and accounting rules follow this trend: 
the Point-in-time estimations recommend in official guidelines of IFRS9 as \cite{IFRS92016} to integrate explanatory economical components in the credit risk assessment process. 
\ares{The EBA guidelines \cite{PDLGD2017}, on LGD downturn, require to identify economic downturn periods to adjust the initial LGD estimations.} Moreover, stress testing described in \cite{Stress2018}, may be based on past economical scenarios.
\\
\\
A credit rating system evaluates the confidence in the ability of the borrower to comply with the credit's terms.
A default probability is associated to each rating, which under the capital rule, Basel regulations (see \cite{Bale2017}), impacts the amount of capital required for a credit.
\\
Such ratings may be generated by internal rating systems (IRB) or issued when it is available, by external rating agencies (like Moody’s, Standard and Poor’s, Fitch Ratings...). 
After the assignment of the initial credit rating, reviews are performed either periodically or based on
market events. In that way an entity's rating may evolve through time according to its health and the economic cycle.
Therefore, predicting the evolution of rating migrations is of primary importance for every financial institution. The migrations of a group of credit entities can be described by transition matrices, defining the probabilities to move from one rating state to another in a given period of time. Given recent evolution in banking supervisory and accounting rules, the challenge is to explain changes in transition probabilities due to changes in the business cycle. 
\\
\\
Factor-based migration models provide a nice framework for capturing migration sensitivities to macro-economic changes. Factor migration models allow transition probabilities to depend on dynamic factors. Two main families of models are usually considered in the credit risk literature~: the ``ordered Probit'' (or structural approach) introduced by \cite{tobin1958estimation}, popularized by \cite{merton1974pricing} and studied for credit ratings , e.g., in \cite{bangia2002ratings}, \cite{feng2008ordered}, \cite{Gagliardini2005}, \cite{nickell2000stability} and the ``multi-state latent factor intensity model'' (or intensity approach) studied, e.g., in \cite{figlewski2012modeling}, \cite{kavvathas2001estimating}, \cite{koopman2008multi}.
This paper focuses on the second approach.
\\
\\
In the basic reduced intensity form model, a credit event corresponds to the first jump time of a Poisson process with a constant hazard rate. The reduced form approach has been widely studied in the credit risk literature, see, e.g., \cite{duffie2007multi}, \cite{jarrow1997markov}...
Nevertheless we can point out a limit of this naive modeling: many studies show that rating migrations' dynamics first exhibit the non-Markovian behavior (migration data exhibit correlation among rating change dates, known as “rating drift”, time-dependent default and transition probabilities, contagion effect ...) that cannot be captured by this model. 
Other papers such as \cite{altman1992implications}, \cite{fledelius2004non} and \cite{hamilton2004rating} highlighted that migration intensities vary over time. In their research, \cite{hamilton2004rating} and \cite{lando2002analyzing} came to the conclusion that the rating transition probabilities depend on whether the bond entered its current rating by an upgrade or a downgrade. \cite{lando2002analyzing} also noticed that the probability to leave a rating category tends to decrease with the time spent at that rating. Above all, \cite{bangia2002ratings}, \cite{nickell2000stability} gave strong evidence that credit risk exposure is considerably affected by the macroeconomic conditions and differ across different economic regimes. The first paper highlighted quantified rating migrations' dependency on the industry, domicile of the obligor and on the stage of the business cycle.
\\
In the factor intensity approach, the migration dynamics of each credit entity is described by a stochastic intensity matrix (or generator matrix) whose components depend on a pool of common factors.
\\
\\
In both models the factors may be considered observable or not.
The second approach has emerged in response to criticisms made against the first. As \cite{Gagliardini2005} pointed out, the risk in selecting covariates lies in excluding other ones which could be more relevant.
\cite{Reda2015} provided an overview of usual modelling and estimation approaches and compared the estimation and predictive performance of each approach on real data. When the underlying factors are unobservable, they adapted a method given in \cite{Gagliardini2005} to represent the considered factor migration model as a linear Gaussian model, and apply a Kalman filter to predict the state of the underlying latent factor. This approximation works on the hypothesis that the transition probabilities' estimator relies on asymptotic normality. This assumption may be too restrictive and typically does not hold when the data set is too small. In this respect, \cite{Reda2015} obtained poor calibration and predictive results using this approximation compared to the estimation performed under the observable factor approach.
\\
\\
Our approach consists in directly filtering the hidden factor given rating transitions' past history. For a bond portfolio, the dynamics of rating migrations can be mathematically represented as a multidimensional counting process, each component representing the cumulative number of transitions from one rating category to another. This framework has been already used in the credit risk literature for other applications:  \cite{frey2012pricing} used a counting process filtering approach to estimate the latent factor given default observation and use this estimation to price credit derivatives.
\ares{
Filtering theory with a counting process has been also applied to credit risk for example in \cite{giesecke2018filtered} and \cite{Leijdekker_Spreij2008}.}
\\
\\
Assuming that the counting process has a latent intensity determined by the hidden factor's state, this project will look into estimating this intensity only using  observations of the counting process.
In our framework, we assume that the unobserved driving factor is given as a finite state Markov chain and rating transitions process as Hidden Markov Chain (HMM).
\ares{
Mixture of Markov Chain (MMC). 
Previous studies already advocated a MMC model to account for stochastic business cycle effect in credit rating migration risk (\cite{fei2012credit}, \cite{frydman2008credit},...). \cite{fei2012credit} demonstrated the efficiency of such approach which resulted in considerably decreasing the capital requirement from BASEL III. They used the trajectory of a two states economic factor (one of contraction and one of expansion) provided by The National Bureau of Economic Research (NBER) to estimate the factor's dynamic. 
However this modeling is totally dependant on the information provided by the institution and might be restrictive. A more reliable alternative is to consider the Markov chain not observable.} 
Hidden Markov Chain modeling (HMM) is a popular approach in credit risk analysis (\cite{ching2009modeling}, \cite{elliott2008hidden}, \cite{elliott2014double}, \cite{thomas2002hidden},...). Among others, \cite{giampieri2005analysis}, used an EM algorithm, the classical Baum-Welch algorithm (introduced in \cite{baum1970maximization}), for estimation of a two-state hidden factor driving  occurrence of defaults. They applied the model to all entities and to different sectors to compare global and industry-specific risks. 
\ares{
\cite{korolkiewicz2008hidden} supposed that a Markov chain governing the \emph{true} credit quality evolution is hidden in \emph{noisy} or incomplete observations represented by credit ratings. As we do in this paper, they used filtering and expected maximization approach to calibrate their model.}
In the same vein \cite{deroose2008reviewing} and \cite{oh2019estimation} identified two hidden states as one of expansion and the other of contraction. The second is the closest study from ours. As we do in this paper, they recently used an extension of the Baum-Welch algorithm adapted to "regime switching hidden Markov model" (RSMC) to propose a forecasting of sovereign credit rating transitions. In a different scope, they also assumed that every rating processes are governed by an unique discrete hidden Markov chain but issued from different trajectories of this Markov chain. Those studies are theoretically different from our models in which a realization of the observable factor is common to every firm. We believe that our approach which rather keeps the dependencies within the observations sample, is more reliable and realistic. Indeed rating entities should be affected by the same realization of the economic factor. This different consideration changes the way to calibrate and to filter totally: our filtering framework uses the whole history of aggregated number of jumps. Furthermore for the sake of interpretability, our approach is more reliable if we want to consider the hidden factor as the universal and shared factor describing the economic cycle. 
\\
\\
\tom{
Rating transitions are usually registered on a daily basis, so that transitions of different entities may be observed at the exact same date. \cite{Bremaud1981} derives a general multivariate counting process filtering formula and then, an application to Markov processes. Nevertheless, its formula holds in continuous time and its application relies on the assumption of no simultaneous jumps in the migration counting processes. The proposed framework can not directly be applied to the context of rating migrations.
}
\ares{
According to many studies like \cite{lando2002analyzing}, using continuous-time analysis of the rating transition data is essential to meaningfully estimate probabilities of rare transitions. 
When those transitions are not directly and indirectly observed in our data set but are still possible, the discrete model might send null values which does not reflect reality.
The continuous-time estimator is not so radical and is able to capture those rare events. Moreover they defended that censoring is handled easily within continuous-time framework. }
\\
\\
\tom{
A discrete-time approach would more relevant with the daily format of the data. \cite{elliott2008hidden} presents a discrete-time filtering framework but this last only holds for Markov processes.
\\
\\
Behind every model mentioned, choosing a continuous or discrete approach is crucial and is a matter of debate. This paper aims to participate to this debate by presenting different results: it present how to adapt continuous filtering framework to be applied to rating transitions context. Furthermore, it proposes a general filtering formula in discrete-time and its version for credit rating application. It assesses and compares the two alternative stochastic migration models, the continuous factor-based intensity approach and its discrete-time version, on their ability to link the rating transition probabilities to an unobservable dynamic risk factor.
}
\ares{
The methods, presented here, consists in filtering the underlying driving factor through the observations of a multivariate point process which counts migration events. 
}
\\
\tom{
The contributions of the paper are both theoretical and practical. 
Two theoretical results are noteworthy: 
we derive a general discrete version of the filtering equation. Then continuous-time and discrete-time formulas are adapted and applied to credit rating migrations context. In particular, we show how one can adapt continuous-time version to a discrete-time phenomenon with the presence of simultaneous jumps. An EM algorithm is extended for both settings to estimate the parameters involved.} 
Applying the recursive equations, we update the filtered factor to forecast rating transitions. Our approach may be considered as a new Point-in-time (PIT) rating transitions modeling which does not use any macro-economic factors.
We assess and compare both approaches on a fictive data set and on a Moody's ratings history [01/2000-05/2021] of a diversified portfolio of 5030 corporate entities. 
To the best of our knowledge, this study is the first attempt to apply and compare both discrete and continuous multivariate counting process filtering to predict future rating transitions.
\\
\\
\tom{
The paper is organised as follows. We present theoretical results, the  derivation of the discrete point process filtering methods and its application to credit migration processes throughout Section \ref{sec:dt-filter}. Section \ref{sec:continuous-filter-article} presents the continuous-time filtering version and its adaptations to discrete-time credit rating environment. The proposed adaptations aim to estimate parameters involved while respecting the different constraints of the models. 
Section \ref{sec:fictiveData}, shows and validates the two filtering results on fictive data. This kind of experiment presents many advantage but is not sufficient to deeply challenge models. Consequently in Section \ref{sec:realData}, we test and compare the two filters on real data sets. Finally Section \ref{sec:conclusion}, presents the conclusions and possible extensions of the paper.
}


